A Survey on Multimodal Benchmarks: In the Era of Large AI Models

The rapid evolution of Multimodal Large Language Models (MLLMs) has brought substantial advancements in artificial intelligence, significantly enhancing the capability to understand and generate multimodal content. As MLLMs advance toward omni-modal perception, reflective self-improvement, unified synthesis, and autonomous agency, evaluation has undergone a fundamental departure from traditional static, task-isolated leaderboards. In this paper, we present a systematic and comprehensive overview of 358 peer-reviewed multimodal benchmarks published between 2024 and 2026. Specifically, we structure this rapidly expanding landscape into five core evaluation pillars, namely understanding, reasoning, generation, trustworthiness and safety, and application, examining their task formulations, capability frontiers, and specialized evaluation metrics across diverse modalities and deployment scenarios. Beyond cataloging individual suites, we review end-to-end dataset construction and quality-control pipelines, and critically analyze key methodological pitfalls governing cross-benchmark comparison validity, including unimodal shortcuts, acausal decision protocols, closed-loop sandbox bottlenecks, and cross-stage biases in LLM-based data synthesis and judging. Building on this analysis, we distill actionable benchmark design blueprints and a pre-release validity checklist to guide reliable evaluation design. We hope that this survey will contribute to the ongoing advancement of MLLM research by offering a comprehensive overview of benchmarking practices and identifying promising directions for future work. An associated GitHub repository collecting the latest papers is available at https://github.com/HKUST-LongGroup/Awesome-MLLM-Benchmarks.

==> figures/reference_positions.tex <==
\@namedef{figpage@survey_map}{1}
\@namedef{figrefs@survey_map}{%
  \figureSection{361.69202}{376.20551}{12.47849}{5.61530}{Bold}{sec:intro}%
  \figureSection{207.76334}{327.90516}{11.18761}{13.98451}{Roman}{sec:understanding_bg}%
  \figureSection{207.76334}{296.92409}{11.18761}{13.98451}{Roman}{sec:understanding_task}%
  \figureSection{308.95009}{300.79673}{11.18761}{5.59380}{Roman}{sec:understanding}%
  \figureSection{207.76334}{256.47659}{11.18761}{13.98451}{Roman}{sec:reasoning_bg}%
  \figureSection{207.76334}{225.49552}{11.18761}{13.98451}{Roman}{sec:reasoning_task}%
  \figureSection{311.74699}{229.36816}{11.18761}{5.59380}{Roman}{sec:reasoning}%
  \figureSection{207.76334}{185.04802}{11.18761}{13.98451}{Roman}{sec:generation_bg}%
  \figureSection{207.76334}{154.06695}{11.18761}{13.98451}{Roman}{sec:generation_task}%
  \figureSection{311.74699}{157.93958}{11.18761}{5.59380}{Roman}{sec:generation}%
  \figureSection{207.76334}{113.61945}{11.18761}{13.98451}{Roman}{sec:trustworthiness_bg}%
  \figureSection{207.76334}{82.63838}{11.18761}{13.98451}{Roman}{sec:trustworthiness_task}%
  \figureSection{311.74699}{86.51101}{11.18761}{5.59380}{Roman}{sec:trustworthiness}%
  \figureSection{207.76334}{42.19088}{11.18761}{13.98451}{Roman}{sec:application_bg}%
  \figureSection{207.76334}{11.20981}{11.18761}{13.98451}{Roman}{sec:application_task}%
  \figureSection{311.74699}{15.08244}{11.18761}{5.59380}{Roman}{sec:application}%
  \figureSection{962.07927}{355.01360}{11.18761}{13.98451}{Roman}{sec:corpus_protocol}%
  \figureSection{889.45822}{337.37160}{11.18761}{13.98451}{Roman}{sec:dataset_collection}%
  \figureSection{871.33670}{319.72960}{11.18761}{13.98451}{Roman}{sec:quality_control}%
  \figureSection{680.72289}{325.75370}{11.18761}{5.59380}{Roman}{sec:holistic_evaluation}%
  \figureSection{859.77413}{259.91893}{11.18761}{13.98451}{Roman}{sec:evolution}%
  \figureSection{957.61653}{228.93786}{11.18761}{13.98451}{Roman}{sec:protocols}%
  \figureSection{950.44912}{197.95680}{11.18761}{13.98451}{Roman}{sec:crossstats}%
  \figureSection{964.17541}{166.97573}{11.18761}{13.98451}{Roman}{sec:patterns}%
  \figureSection{680.72289}{187.19948}{11.18761}{5.59380}{Roman}{sec:cross}%
  \figureSection{680.72289}{74.89311}{11.18761}{5.59380}{Roman}{sec:direction}%
  \figureSection{714.21617}{26.80792}{12.47849}{12.26635}{Bold}{sec:conclusions}%
}
\@namedef{figpage@understanding_map}{2}
\@namedef{figrefs@understanding_map}{%
  \figureSection{281.89389}{502.18444}{13.60896}{27.21786}{Roman}{sec:u1_single_item}%
  \figurePaper{418.89758}{476.30108}{13.78322}{22.96282}{Roman}{zhang2024q-bench}%
  \figurePaper{418.89765}{457.35190}{13.78322}{22.96282}{Roman}{tong2024mmvp}%
  \figurePaper{418.89754}{438.40272}{13.78322}{22.96282}{Roman}{fu2025ocrbenchv2}%
  \figurePaper{418.89761}{419.45354}{13.78322}{22.96282}{Roman}{amaduzzi2024LLaNA}%
  \figureSection{281.89389}{353.17496}{13.60896}{27.21786}{Roman}{sec:u2_contextual}%
  \figurePaper{421.88516}{327.73990}{11.99000}{19.97537}{Roman}{luo2024codis}%
  \figurePaper{421.88520}{308.79072}{11.99000}{19.97537}{Roman}{song2024milebench}%
  \figurePaper{421.88516}{289.84154}{11.99000}{19.97537}{Roman}{du2025mir}%
  \figurePaper{415.89023}{270.89235}{11.99000}{25.97038}{Roman}{zong2024VL-ICLBench}%
  \figureSection{281.89389}{204.16549}{13.60896}{27.21786}{Roman}{sec:u3_temporal}%
  \figurePaper{419.78873}{178.41584}{13.24834}{22.07177}{Roman}{liu2024TempCompass}%
  \figurePaper{413.16458}{159.46666}{13.24834}{28.69595}{Roman}{zhang2026timelensbench}%
  \figurePaper{413.16458}{140.51747}{13.24834}{28.69595}{Roman}{li2025ovobench}%
  \figureSection{281.89389}{74.10520}{13.60896}{27.21786}{Roman}{sec:u4_cross_signal}%
  \figurePaper{413.84682}{48.43430}{12.93335}{28.01365}{Roman}{han2025camer}%
  \figurePaper{420.31350}{29.48511}{12.93335}{21.54697}{Roman}{yang2025avut}%
  \figurePaper{413.84682}{10.53593}{12.93335}{28.01365}{Roman}{chen2024mcub}%
}
\@namedef{figpage@reasoning_map}{3}
\@namedef{figrefs@reasoning_map}{%
  \figureSection{281.51966}{531.91215}{13.60896}{27.21786}{Roman}{sec:r1_conclusion}%
  \figurePaper{415.95899}{506.48504}{11.95821}{25.90148}{Roman}{wang2024measuring}%
  \figurePaper{415.95895}{487.53586}{11.95821}{25.90148}{Roman}{ma20253dsrbench}%
  \figurePaper{415.95895}{468.58668}{11.95821}{25.90148}{Roman}{chen2024m3cot}%
  \figureSection{281.51966}{342.85100}{13.60896}{27.21786}{Roman}{sec:r2_grounded}%
  \figurePaper{412.46717}{317.02084}{13.57037}{29.39347}{Roman}{zhou2025refspatialbench}%
  \figurePaper{412.46703}{298.07166}{13.57037}{29.39347}{Roman}{yan2024revos}%
  \figurePaper{412.46710}{279.12248}{13.57037}{29.39347}{Roman}{wang2026treebench}%
  \figureSection{281.51966}{212.79070}{13.60896}{27.21786}{Roman}{sec:r3_trace}%
  \figurePaper{416.94684}{187.47760}{11.50212}{24.91363}{Roman}{jiang2025mmecot}%
  \figurePaper{416.94691}{168.52842}{11.50212}{24.91363}{Roman}{thawakar2025vrcbench}%
  \figurePaper{416.94691}{149.57924}{11.50212}{24.91363}{Roman}{shi2026mathcanvasbench}%
  \figureSection{281.51966}{76.27046}{13.60896}{27.21786}{Roman}{sec:r4_judgment}%
  \figurePaper{416.21284}{50.87265}{11.84100}{25.64759}{Roman}{wu2025visco}%
  \figurePaper{416.21277}{31.92347}{11.84100}{25.64759}{Roman}{chen2024mllmasajudge}%
  \figurePaper{416.21280}{12.97429}{11.84100}{25.64759}{Roman}{huang2024VLKEB}%
}
\@namedef{figpage@generation_map}{4}
\@namedef{figrefs@generation_map}{%
  \figureSection{281.89389}{452.22750}{13.60896}{27.21786}{Roman}{sec:g1_verbal}%
  \figurePaper{414.42899}{426.62379}{12.66459}{27.43151}{Roman}{ding2025mmifeval}%
  \figurePaper{414.42903}{407.67461}{12.66459}{27.43151}{Roman}{qian2024mia}%
  \figurePaper{414.42906}{388.72543}{12.66459}{27.43151}{Roman}{lei2025godbench}%
  \figureSection{281.89389}{322.16721}{13.60896}{27.21786}{Roman}{sec:g2_executable}%
  \figurePaper{413.99290}{296.51317}{12.86591}{27.86757}{Roman}{yang2025chartmimic}%
  \figurePaper{413.99297}{277.56399}{12.86591}{27.86757}{Roman}{si2025design2code}%
  \figurePaper{420.42586}{258.61481}{12.86591}{21.43461}{Roman}{yin2026blenderbench}%
  \figureSection{281.89389}{133.10606}{13.60896}{27.21786}{Roman}{sec:g3_media}%
  \figurePaper{413.73957}{107.42275}{12.98288}{28.12100}{Roman}{zhao2025risebench}%
  \figurePaper{420.23103}{88.47360}{12.98288}{21.62954}{Roman}{pang2025paper2poster}%
  \figurePaper{413.73964}{69.52442}{12.98288}{28.12100}{Roman}{arora2025talkingturns}%
}
\@namedef{figpage@trustworthiness_map}{5}
\@namedef{figrefs@trustworthiness_map}{%
  \figureSection{281.13858}{464.28607}{13.60896}{27.21786}{Roman}{sec:t1_hallucination}%
  \figurePaper{415.48763}{438.80454}{12.17586}{26.37290}{Roman}{kaul2024throne}%
  \figurePaper{415.48760}{419.85535}{12.17586}{26.37290}{Roman}{cheng2025simplevqa}%
  \figurePaper{415.48756}{400.90617}{12.17586}{26.37290}{Roman}{ye2025eyesearsdisagree}%
  \figureSection{281.13858}{334.22578}{13.60896}{27.21786}{Roman}{sec:t2_safety}%
  \figurePaper{412.57460}{308.40803}{13.52070}{29.28584}{Roman}{ying2026safebench}%
  \figurePaper{412.57460}{289.45885}{13.52070}{29.28584}{Roman}{zhu2025moho}%
  \figurePaper{412.57463}{270.50967}{13.52070}{29.28584}{Roman}{li2024MMUBench}%
  \figureSection{281.13858}{204.16549}{13.60896}{27.21786}{Roman}{sec:t3_robustness}%
  \figurePaper{415.94777}{178.73708}{11.96339}{25.91269}{Roman}{liu2024MMR}%
  \figurePaper{415.94781}{159.78790}{11.96339}{25.91269}{Roman}{ye2024mm}%
  \figurePaper{415.94777}{140.83872}{11.96339}{25.91269}{Roman}{luo2024JailBreakV-28K}%
  \figureSection{281.13858}{74.10520}{13.60896}{27.21786}{Roman}{sec:t4_diagnostics}%
  \figurePaper{415.18072}{48.58826}{12.31750}{26.67967}{Roman}{mickus2026sheep}%
  \figurePaper{415.18076}{29.63908}{12.31750}{26.67967}{Roman}{li2025vlrewardbench}%
  \figurePaper{415.18072}{10.68990}{12.31750}{26.67967}{Roman}{ye2025loki}%
}
\@namedef{figpage@application_map}{6}
\@namedef{figrefs@application_map}{%
  \figureSection{281.89389}{905.28514}{13.60896}{27.21786}{Roman}{sec:app_group1}%
  \figurePaper{411.63725}{879.35927}{13.95349}{30.22332}{Roman}{cheng2024screenspot}%
  \figurePaper{411.63729}{860.41009}{13.95349}{30.22332}{Roman}{gou2025mind2web2}%
  \figurePaper{411.63729}{841.46091}{13.95349}{30.22332}{Roman}{paglieri2025balrog}%
  \figureSection{281.89389}{775.22485}{13.60896}{27.21786}{Roman}{sec:app_group1}%
  \figurePaper{416.77601}{749.89205}{11.58102}{25.08449}{Roman}{wei2025mineanybuild}%
  \figurePaper{416.77608}{730.94287}{11.58102}{25.08449}{Roman}{yang2025embodiedbench}%
  \figurePaper{416.77601}{711.99369}{11.58102}{25.08449}{Roman}{quevedo2026worldgym}%
  \figurePaper{416.77601}{693.04451}{11.58102}{25.08449}{Roman}{wang2025omnidrive}%
  \figureSection{281.89389}{626.21538}{13.60896}{27.21786}{Roman}{sec:app_group2}%
  \figurePaper{414.09709}{600.57339}{12.81782}{27.76341}{Roman}{zuo2025medxpertqa}%
  \figurePaper{414.09709}{581.62421}{12.81782}{27.76341}{Roman}{chen2025slidebench}%
  \figurePaper{414.09709}{562.67503}{12.81782}{27.76341}{Roman}{jin2026diningbench}%
  \figureSection{281.89389}{496.15512}{13.60896}{27.21786}{Roman}{sec:app_group2}%
  \figurePaper{411.63729}{470.22918}{13.95349}{30.22332}{Roman}{li2024vrsbench}%
  \figurePaper{411.63729}{451.28000}{13.95349}{30.22332}{Roman}{zhou2025urbench}%
  \figurePaper{411.63729}{432.33081}{13.95349}{30.22332}{Roman}{shinoda2025agrobench}%
  \figureSection{281.89389}{366.09486}{13.60896}{27.21786}{Roman}{sec:app_group2}%
  \figurePaper{417.28459}{340.82073}{11.34622}{24.57588}{Roman}{liu2026moscibench}%
  \figurePaper{422.95769}{321.87155}{11.34622}{18.90278}{Roman}{starace2025paperbench}%
  \figurePaper{417.28462}{302.92237}{11.34622}{24.57588}{Roman}{alampara2025macbench}%
  \figurePaper{422.95765}{283.97319}{11.34622}{18.90278}{Roman}{yang2025swebenchmultimodal}%
  \figureSection{281.89389}{210.62544}{13.60896}{27.21786}{Roman}{sec:app_group2}%
  \figurePaper{414.47865}{185.02740}{12.64166}{27.38188}{Roman}{su2025essayjudge}%
  \figurePaper{414.47858}{166.07822}{12.64166}{27.38188}{Roman}{shi2025mumatom}%
  \figurePaper{414.47858}{147.12904}{12.64166}{27.38188}{Roman}{jia2025aicd}%
  \figureSection{281.89389}{64.63054}{13.60896}{27.21786}{Roman}{sec:app_group2}%
  \figurePaper{412.15269}{38.76411}{13.71550}{29.70770}{Roman}{luo2025finmme}%
  \figurePaper{412.15262}{19.81492}{13.71550}{29.70770}{Roman}{wang2025ecombench}%
}


==> layout_macros.tex <==
% Layout and figure helper macros for the survey manuscript.
\usepackage{tabularx}
\usepackage{placeins}

\makeatletter
\input{figures/reference_positions.tex}
\definecolor{figuresectionink}{HTML}{781D7D}
\definecolor{figurepaperink}{HTML}{654479}
\newsavebox{\figureartbox}
\newcommand{\figurefaceRoman}{\rmfamily}
\newcommand{\figurefaceBold}{\sffamily\bfseries}
\newcommand{\figureSection}[6]{%
  \put(#1,#2){\fontsize{#3\unitlength}{#3\unitlength}\selectfont\csname figureface#5\endcsname
    \hyperref[#6]{\textcolor{figuresectionink}{\resizebox{#4\unitlength}{!}{\ref*{#6}}}}}}
\newcommand{\figurePaper}[6]{%
  \put(#1,#2){\fontsize{#3\unitlength}{#3\unitlength}\selectfont\csname figureface#5\endcsname
    \hyperlink{cite.#6}{\textcolor{figurepaperink}{\resizebox{#4\unitlength}{!}{%
      \begin{NoHyper}\@fileswfalse\cite{#6}\end{NoHyper}}}}}}
\newcommand{\chaptergraphic}[2][]{%
  \begingroup
  \edef\figurestem{#2}%
  \sbox{\figureartbox}{\includegraphics[page=\csname figpage@\figurestem\endcsname,#1]{figures/reference_art.pdf}}%
  \setlength{\unitlength}{\dimexpr\wd\figureartbox/1000\relax}%
  \leavevmode\hbox{\usebox{\figureartbox}\kern-\wd\figureartbox
    \rlap{\smash{\begin{picture}(0,0)\csname figrefs@\figurestem\endcsname\end{picture}}}%
    \kern\wd\figureartbox}%
  \endgroup}
\makeatother

\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@dblfptop}{0pt}
\setlength{\@fpsep}{7pt}
\setlength{\@dblfpsep}{7pt}
\makeatother
\setlength{\floatsep}{8pt plus 3pt minus 2pt}
\setlength{\dblfloatsep}{8pt plus 3pt minus 2pt}
\setlength{\textfloatsep}{9pt plus 4pt minus 2pt}
\setlength{\dbltextfloatsep}{9pt plus 4pt minus 2pt}
\setcounter{dbltopnumber}{4}
\setcounter{topnumber}{2}

\renewcommand{\dbltopfraction}{.96}
\renewcommand{\topfraction}{.96}
\renewcommand{\textfraction}{.03}
\renewcommand{\floatpagefraction}{.97}
\renewcommand{\dblfloatpagefraction}{.97}
\flushbottom

